Context-Aware Crowd Counting

State-of-the-art methods for counting people in crowded scenes rely on deep networks to estimate crowd density. They typically use the same filters over the whole image or over large image patches. Only then do they estimate local scale to compensate for perspective distortion. This is typically achieved by training an auxiliary classifier to select, for predefined image patches, the best kernel size among a limited set of choices. As such, these methods are not end-to-end trainable and restricted in the scope of context they can leverage. In this paper, we introduce an end-to-end trainable deep architecture that combines features obtained using multiple receptive field sizes and learns the importance of each such feature at each image location. In other words, our approach adaptively encodes the scale of the contextual information required to accurately predict crowd density. This yields an algorithm that outperforms state-of-the-art crowd counting methods, especially when perspective effects are strong.

==> geo_diff.tex <==
% !TEX root = ../ms.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
      \begin{subfigure}{.3\textwidth}
        \centering
        \includegraphics[width=.9\linewidth]{world_geo_1.jpg}
        \label{fig:world_geo_1}
      \end{subfigure}%
      \begin{subfigure}{.3\textwidth}
          \centering
          \includegraphics[width=.9\linewidth]{world_geo_2.jpg}
          \label{fig:world_geo_2}
        \end{subfigure}%
      \begin{subfigure}{.3\textwidth}
          \centering
          \includegraphics[width=.9\linewidth]{world_geo_3.jpg}
          \label{fig:world_geo_3}
        \end{subfigure}

        \begin{subfigure}{.3\textwidth}
          \centering
          \includegraphics[width=.9\linewidth]{venice_geo_1.jpg}
          \label{fig:venice_geo_1}
        \end{subfigure}%
        \begin{subfigure}{.3\textwidth}
            \centering
            \includegraphics[width=.9\linewidth]{venice_geo_2.jpg}
            \label{fig:venice_geo_2}
          \end{subfigure}%
        \begin{subfigure}{.3\textwidth}
            \centering
            \includegraphics[width=.9\linewidth]{venice_geo_3.jpg}
            \label{fig:venice_geo_3}
          \end{subfigure}
  \caption{Visualization of geometry information quality. First rows are images from \textit{WorldExpo'10} dataset while images of the second row are from \textit{Venice} dataset. On each image, a ellipse is shown in red, which is a circular with radius of 1 meter in physical world and projected to image plane based on provided geometry information of each dataset. It clearly shows that geometry information of \textit{Venice} dataset is much more accurate since (1) the distortion of ellipse in \textit{Venice} dataset follows the same change as scene geometry while it is not the case for \textit{WorldExpo'10} dataset. (2) The radius of 1 meter is consistent among different scenes while in \textit{WorldExpo'10} it varies a lot.}
  \label{fig:geo_diff}
  \end{figure*}


==> sf.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
\centering
        \includegraphics[width=.9\linewidth]{sf_pdf.pdf}
  \vspace{-3mm}
  \caption{ {\bf Scale aware features.} The Input RGB image is fed to a convolutional network whose first 10  layers are those of \textit{VGG-16}. The resulting local features are grouped in blocks of several size by average pooling followed by 1$\times$1 convolutional layer. They are then up-sampled back to the original feature size to form the contrast features. The contrast features are the difference local features and context features.}
  \label{fig:sf}
 \end{figure*}
